Understanding Contrastive Learning Requires Incorporating Inductive Biases

Contrastive learning is a popular form of self-supervised learning that encourages augmentations (views) of the same input to have more similar representations compared to augmentations of different inputs. Recent attempts to theoretically explain the success of contrastive learning on downstream classification tasks prove guarantees depending on properties of {\em augmentations} and the value of {\em contrastive loss} of representations. We demonstrate that such analyses, that ignore {\em inductive biases} of the function class and training algorithm, cannot adequately explain the success of contrastive learning, even {\em provably} leading to vacuous guarantees in some settings. Extensive experiments on image and text domains highlight the ubiquity of this problem -- different function classes and algorithms behave very differently on downstream tasks, despite having the same augmentations and contrastive losses. Theoretical analysis is presented for the class of linear representations, where incorporating inductive biases of the function class allows contrastive learning to work with less stringent conditions compared to prior analyses.

==> B-experiments.tex <==
\section{Experiments}
\label{sec:appendix-experiments}

In this section, we provide additional notes, tables, and figures on the experiments.

\subsection{Synthetic experiments: hypercube example}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{media/synth_large.pdf}
    \caption{Full plots for the synthetic experiments.}
    \label{fig:synth-large}
\end{figure}

\subsection{CIFAR-10 + SimCLR experiments}

\subsection{Language experiments}


==> _3-pitfalls.tex <==
% !TEX root = main.tex

\section{Pitfalls of function class agnostic analyses}
\label{sec:pitfalls}



\iffalse

To expand upon the above discussion, consider the SOTA theory for contrastive learning from \citet{haochen2021provable}.
\highlight{rephrase so that it doesn't seem like we're just criticizing this one paper. \sg{Yes, please!}}
Their formalization of (1) requires sufficient overlap in augmentation distributions of inputs from the same downstream class but low overlap between inputs from different classes.
For such augmentations, they show that a representation $f$ that approximately minimizes a contrastive loss $\Lcont$ will have downstream error upper bounded by $\gO\left(\Lcont(f) - \Lcont(f^{*})\right)$, where $f^{*}$ is a minimizer of $\Lcont$, thus justifying minimizing $\Lcont$.
Notably, the best bound is obtained for all minimizers of the contrastive loss.
This is also a common theme for many other analysis: under some assumptions on augmentations, prove that the minimizer of a contrastive loss will do well on the downstream task.
This raises many intriguing questions:
\begin{itemize}[leftmargin=*]
  \item Are we anywhere close to minimizing $\Lcont$ in practice? Do we even need $\Lcont(f) - \Lcont(f^{*})$ to be small to guarantee good downstream performance?
  \item Can guarantees be shown for the best representation in function class instead of unconstrained minimizers of $\Lcont$, especially when $\min_{f\in\gF} \Lcont(f) \neq \Lcont(f^{*})$? Can they be better than those that ignore function class?
  \item Can we show guarantees under weaker assumptions on augmentations if we incorporate function class biases?
\end{itemize}

In the rest of the paper we address many of the above questions and answer them in the positive, guided by simple examples, theoretical results, experiments on standard datasets and simulations. \highlight{Rough list below}



\begin{itemize}[leftmargin=*]
    \item Simple Boolean warm-up hypercube  example in \Cref{sec:} that succinctly highlights many of the above points, supported by simulation experiments.
    \highlight{The main takeaway is summarized in \Cref{table:hypercube}: different function classes (MLP, linear, lookup table) can have very different behaviors and so can different algorithms (Adam w/ and w/o weight decay). There exist good and bad minimizers of the contrastive loss. Can get better guarantees despite (because of) minimizer in class and not unconstrained minimizer.}
    \item Some theory: lower bound for inductive bias agnostic analyses in the case where augmentation distributions do not overlap.
    Analysis for a general case of linear representation function class, that can recover analysis from \citet{haochen2021provable} as a special case.
    \highlight{Guarantees can be shown even in non-overlapping augmentation settings}.
    \item Experiments on CIFAR-10 with ResNet and vision transformer (ViT).
    With weaker augmentations, ViT has a worse CL vs Acc curve than ResNet, but gap reduces as augmentations get stronger.
    Hash experiment, where ViT can pick up on hash but ResNet cannot always.
\end{itemize}

\fi




\ns{Main plan is to describe/formalize a setting that is close to what is happening practice and where not incorporating function class bias can be egregious!}

\begin{enumerate}
    \item \ns{Optional} Describe state-of-the-art result from \cite{} for spectral contrastive learning.
    What properties do they use to show guarantees.
    \item Introduce non-overlapping augmentation distribution setting. Motivate it intuitively and why it is especially relevant for contrastive learning with data augmentations.
    \item Present experimental evidence through the augmentation classification accuracy being close to 100\%.
    Connection of classification error to blow up term.
    \ns{Optional} May be even the MD5 hash experiment, to show that minor changes to the augmentation distribution that makes it non-overlapping still leads to successful contrastive learning.
    \item Perhaps present the Gaussian examples where the overlap is exponentially small or 0, to highlight simple instances of this case.
    \item Show a lower bound on function class agnostic analyses for the non-overlapping setting, for SimCLR and spectral losses as a proposition.
\end{enumerate}




%%%%%% Subsection
\subsection{Spectral Contrastive Learning / Intuition for failure mode}
\label{sec:spectral_cl}
\ns{Optional}

Can first describe the results from \cite{} in more detail.
Discuss that this bound is pretty much state-of-the-art in terms of assumptions required to show such a transfer bound.
The bound strongly depends on the there being overlap between augmentation distributions, more so among inputs from the same class.
This can help identify when the bound is vacuous: when graph is disconnected-ness assumption or has at least $k$ connected components.
Motivates non-overlapping augmentation distributions.







%%%%%% Subsection
\subsection{Non-overlapping augmentation distribution}
\label{sec:non_overlapping}

Setting where augmentation distributions between different inputs have no overlap at all.
This makes more sense for data augmentations where the change to an input may not be large enough for the distributions to overlap.
Note that this almost by definition makes the data augmentation ``label'' preserving, since there is no ambiguity in the label of an augmentation if the same is true for the original input.
Some experimental evidence that augmentations used in practice on images are not too overlapping.

\ns{Something about BYOL and trivial solutions?}




%%%%%% Subsection
\subsection{Lower bound for function class agnostic analyses}
\label{sec:lower_bound}

While we showed that non-overlapping distribution lends the bound from \cite{} vacuous, the issue goes beyond that.m

==> nlp-exp-backup.tex <==
We use Wiki3029 which is a text classification dataset introduced by~\citet{arora2019theoretical}. The downstream task here is to simply predict the class for a given text. 
We preprocess the data to tokenize every text and split the dataset into a train, validation, and a test split. Please see Appendix~\ref{sec:apx_exps} for details.

Compared to vision, there is relatively less study of augmentations for text. We consider four simple augmentations for our study: (i) \emph{Drop}: randomly drop 15\% tokens but keep the order of remaining tokens, (ii) \emph{Drop+Permute}: randomly drop 15\% tokens and randomly permute the remaining tokens, (iii) \emph{Split}: randomly return either the left half or right half of the text, and (iv) \emph{Split+Full}: randomly return from the full text, its left half, or its right half.
%\vspace{-2ex}\begin{itemize}[leftmargin=*,noitemsep]
 %   \item \textbf{Drop:} Randomly drop 85\% tokens but keep the order of remaining tokens.
  %  \item \textbf{Drop+Permute:} Randomly drop 85\% tokens but randomize the order of remaining tokens.
   % \item \textbf{Split:} Randomly return either the left half or right half of the text.
    %\item \textbf{Split+Full:} Randomly return from the full text, its left half, and its right half.
%\end{itemize}

We evaluate three models on this dataset. The first is a simple Bag-of-Word ($\bow$) model that learns a single word embedding matrix and returns the average word embedding of tokens in the text. The second model is Gated Recurrent Unit ($\gru$), which is a recurrent neural network~\cite{chung2014empirical}. And the last is $\transformers$~\citep{vaswani2017attention} which are state-of-the-art neural networks for text domain. Both $\gru$ and $\transformers$, map a text to a sequence of hidden representations with each token associated with a single hidden representation. For both models, we return the average hidden representations of tokens in the text. We follow the SimCLR pipeline for training and evaluating these models. See Appendix~\ref{sec:apx_exps} for details on the experimental setup and hyperparameters.

Figure~\ref{fig:text_experiments} shows training curves relating the validation loss for contrastive learning and the top-10 test classification accuracy on the downstream task for two augmentation types. We evaluate the model at the end of each epoch of contrastive learning, on both the contrastive learning task and the downstream task. Please see Appendix~\ref{sec:apx_exps} for results on the other two augmentations.

We observe that, in general, $\bow$ performs the best on downstream classification task while doing somewhat worse on the contrastive learning task. For the drop augmentation type, $\gru$ fails to solve the downstream task while achieving lower contrastive learning loss. Further, in strong support of our theoretical claims, the downstream accuracy of $\gru$ decreases as its contrastive learning loss decreases. This cannot be explained by previous transfer bound results. We believe that this maybe due to $\gru$ being a more expressive model that captures word order, while the downstream task is somewhat oblivious to word order. This is further elucidated by results on drop+permute augmentations where $\gru$ matches the performance of $\bow$. Finally, $\transformers$ performs poorly on the downstream task while doing quite well on the contrastive learning task for both augmentations. We believe that this maybe due to inherent complexity of $\transformers$ that requires more data to train accurately.

% \cz{pithy intro goes here} Next, we examine the same questions in the text domain. \cz{todo discuss/cite text rep learning papers}

% Datasets: Wiki-3029, AG News, DBPedia

% Augmentations: Random drop (+ permute)

% Architectures: BOW, GRU (1/2 layers), Transformers (w and w/o pos encoding)

% - Transfer plots and collapse

% GRU (and may Transformers) make the contrastive loss low but has bad downstream. Continuous-bag-of-words has worse contrastive loss but good downstream, on Wiki-3029, AG News DBPedia. Table \Cref{table:nlp_results} and transfer plots in \Cref{fig:nlp_transfer}












\paragraph{Experimental Setup.} We evaluate on the Wiki3029 dataset~\cite{arora2019theoretical}. This dataset contains 3029 classes and each class contains 200 lines of text. Each class denotes a Wikipedia article and the 200 liens of text were taken from the body of the article. We split the dataset into a training set, a validation set, and a test set. The training set contains 64\% of the data with 128 examples from each class. the validation set contains 16\% of the data with 32 examples from each class. Finally, the test set contains the remaining 20\% of the dataset with 40 examples from each class. The downstream evaluation task is to simply predict the class given the text. We process each line of text as follows. We first use a NLTK tokenizer to tokenize the text. We replace each token that occurs less than 50 times in the dataset with a special ${\tt UNK}$. This gives us a vocabulary size of 15,679. If a token sequence is of length more than 60, we then trim it to its first 60 tokens. This does not cause significant issue since only $\approx 1.92\%$ of the data has text with more than 60 tokens. 

We perform contrastive learning similar to SimCLR. We train the model in epochs. In each epoch, we first sample pairs of augmentation for 50,000 randomly chosen pieces of text in the training dataset. We then perform a single pass over this dataset and minimize the SimCLR contrastive learning loss. We normalize the representations to unit norm when computing the SimCLR loss. The downstream evaluation task is to simply predict the class given the text. Formally, given a batch $\{(x_i, x'_i)\}_{i=1}^B$ of pairs of augmentation $(x_i, x'_i)$ we perform a single update of Adam to minimize the following loss:

\begin{equation}
\label{eqn:simclr_objective}
    L = -\frac{1}{2B} \sum_{i=1}^n \frac{w(x_i, x'_i)}{\sum_{j=1}^n w(x_i, x'_j) + \sum_{j=1, j\ne i}^n w(x_i, x_j)} -\frac{1}{2B} \sum_{i=1}^n \frac{w(x_i, x'_i)}{\sum_{j=1}^n w(x'_i, x_j) + \sum_{j=1, j\ne i}^n w(x'_i, x'_j)},
\end{equation}
where $w(x, x') = \exp\left(\frac{f(x)^\top f(x')}{\|f(x)\|_2\|f(x')\|_2}\right)$.

At the start of contrastive learning, we create a held-out validation set of pairs of augmentation sampled for 10,000 randomly chosen examples from the original validation set. At the end of each epoch of contrastive learning, we evaluate the model on this held-out validation set by computing the SimCLR loss. We also train a linear classifier to evaluate the model on the downstream classification task. During the linear classificatiion task, we keep the encoder model fixed.

We train the linear classifier on the training set in epochs and use Adam optimization with gradient clip. During the downstream training, we evaluate the model at the end of epoch on the validation set and report the linear classifier with the best validation loss. We stop training if the best validation loss does not improve for $\kappa$ consecutive epochs where $\kappa$ is the patience hyperparameter, or if we hit a maximum number of epochs. 

We list hyperparameter values in Table~\ref{table:hyperparameters_nlp}.

\begin{table*}[!h]
    \centering
    \begin{tabular}{c|c}
         \hline
         \textbf{Hyperparameters} & \textbf{Values} \\
         \hline 
         Max epoch & 100\\
         Learning rate for contrastive learning & 0.001\\
        Learning rate for downstream linear classification & 0.01\\
         Patience & 10 \\
         Batch size & 256\\
         Representation dimension & 768\\
         Gradient clipping norm & 2.5\\
         \hline
    \end{tabular}
    \caption{Hyperparameter values for experiments on Wiki3029. Unless specified, the same hyperparameter value is used for both contrastive learning and the downstream classification task.}
    \label{table:hyperparameters_nlp}
\end{table*}

\paragraph{Model Details.} We evaluate three models on the Wiki3029 task. All models encode a given text to a 768 dimensional vector. The first model is a bag of word ($\bow$) that trains a word embedding matrix and simply returns the average word embedding of tokens in the text. The second is Gated Recurrent Unit ($\gru$) that is a recurrent neural network that applies a function $\psi$ to map the tokenized text $x = (x_i)_{i=1}^n$ to a sequence of hidden representations $\{h_i\}_{i=1}^n$ with $h_i = \psi(x_i, h_{i-1})$ and $h_0$ is the 0 vector. This model returns the average of hidden representations $\nicefrac{1}{n}\sum_{i=1}^n h_i$. Specifically, we use a $\gru$ model that has 1 layer, 300 dimensional word embedding, and uses a dropout of 0.3.  Lastly, we use $\transformers$ which are state-of-the-art architectures for text problems. Similar to $\gru$, the $\transformers$ map a tokenized sequence $x = (x_i)_{i=1}^n$ to a sequence of hidden representations $(h_i)_{i=1}^n$. In this case as well, we return the average hidden representation $\nicefrac{1}{n}\sum_{i=1}^n h_i$. We use a 4 layer transformer, with 128 dimensional representation, and 4 attention heads. After the final transformer layer, we project the 128 dimensional vector to 768 using a single matrix multiplication.

\begin{table*}[!h]
    \centering
    \begin{tabular}{c|c}
         \hline
         \textbf{Hyperparameters} & \textbf{Values} \\
         \hline 
         Max epoch & 100\\
         Learning rate for contrastive learning & 0.001\\
        Learning rate for downstream linear classification & 0.01\\
         Patience & 10 \\
         Batch size & 256\\
         Representation dimension & 768\\
         Gradient clipping norm & 2.5\\
         \hline
    \end{tabular}
    \caption{Hyperparameter values for experiments on Wiki3029. Unless specified, the same hyperparameter value is used for both contrastive learning and the downstream classification task.}
    \label{table:hyperparameters_nlp}
\end{table*}

All our models are implemented in PyTorch and trained on a V100 GPU clusters. The training time for a single experiment takes anywhere from 30min to 2hr. 

\paragraph{Results on Split and Split+Full augmentations.} We present results on these two augmentations in Figure~\ref{fig:text_experiments_remaining}. These results are similar to the performance on the drop augmentation. We observe that $\bow$ achieves the best downstream performance while achieving a higher contrastive loss, whereas the more expressive models achieve better contrastive loss but poorer downstream accuracy. In particular, the downstream accuracy of $\gru$ decrease as its validation loss on the contrastive learning task decreases. This is a strong evidence for our work and shows the importance of understand the inherent bias of the model. 

\begin{figure}[t!]
    \centering
    \includegraphics[scale=0.5]{ICML2022/media/plot_split_top_10_accuracy.pdf}
     \includegraphics[scale=0.5]{ICML2022/media/plot_split_or_full_top_10_accuracy.pdf}
    \caption{Top-10 test classification accuracy against contrastive validation loss on Wiki3029 for various augmentations and models.}
    \label{fig:text_experiments_remaining}
\end{figure}

%Architectures: BOW, GRU (1/2 layers), Transformers (w and w/o pos encoding)

%- Transfer plots and collapse

%GRU (and may Transformers) make the contrastive loss low but has bad downstream. Continuous-bag-of-words has worse contrastive loss but good downstream, on Wiki-3029, AG News DBPedia. Table \Cref{table:nlp_results} and transfer plots in \Cref{fig:nlp_transfer}






==> paper_elements.tex <==
\subsection{Paper elements}



\paragraph{Hypercube example:}
Simple example that highlights the main points.
Mostly experimental, some parts are justified by the general analysis for linear representations that shows up later.
Below is the simplest such example

Inputs are vertices of the hypercube $\{\pm 1\}^{D}$, downstream label is a linear in the first $k\ll D$ coordinates: $y = w^{\top} \bar{x}[:k], w\in\R^{k}$. Augmentation $x$ of input $\bar{x}$ is obtained by sampling $\tau \in [0, 1]$ and downscaling label agnostic coordinates by $\tau$; so $x[:k] = \bar{x}[:k]$ and $x[k:] = \tau ~\bar{x}[k:]$\footnote{this can be generalized to only downscaling random subsets of $\bar{x}[k:]$, analogous to randomly downscaling different aspect of an image like grayness, sharpness}

First $k$ coordinates are not affected while others are scaled down, so it intuitively seems like contrastive learning should help. But it's easy to see that this is the "non-overlapping" setting, since the original input $\bar{x}$ can be perfectly recovered from its augmentation $x$: $\bar{x} = sign(x)$.
This lets us construct minimizers of the contrastive loss that basically have 50\% accuracy on downstream.

However if the representation class is linear, then contrastive learning provably does well on downstream task. In experiments, even an MLP representation does better than random guessing on the downstream task. For MLP the algorithm also matters (weight decay or not). In both cases we do not learning the absolute minimizer of $\Lcont$.
\Cref{table:hypercube} summarizes the results of simulation experiments on this example.


\highlight{
TODOs:

- Figure out the most convincing form of this example. (current example is good enough)

Experiments

-- Rerun Table 1 with std dev.

-- Downstream task that is quadratic in $x[:k]$ instead of linear

-- Aug clf experiment?
}


\paragraph{Theory:}
Some of the above phenomena can be theoretically explained.
Lower bound: Show existence of bad minimizers in the non-overlapping augmentation setting, for multiple contrastive losses, through a probabilistic argument.
Upper bound: Show guarantees for spectral loss with linear representation class, and how it can instantiated to give non-trivial guarantees for the non-overlapping setting.

\highlight{
TODOs:

- Write down the lower bound for non-overlapping

- Finish the low-rank linear representation result. Include topic modeling example?

- (Optional) Include bounded norm linear representation result? 
}

\paragraph{CIFAR-10 experiments:}
Two main questions:

- Are we finding a minimizer of the contrastive loss in practice? Hash experiment suggests that we might not be.
Encode a hash of the original image into augmentations such that it becomes a non-overlapping setting. Running SimCLR on this leads to a ResNet still getting high accuracy, while ViT will make the contrastive loss much smaller but have terrible downstream performance

- Do different classes ``transfer'' differently? ViT v/s ResNet experimets for various augmentation strengths suggest that ResNets transfer better for weaker augentations, but the gap vanishes as augmentations get stronger.

\highlight{
TODOs:

- Run 3 kinds of hash experiments with ResNet and ViT

- Run ViT and ResNet for various scalings of random cropping for contrastive loss v/s downstream accuracy scatter plots

- Augmentation classification experiment for various scales

- \dipendra{Wiki-3029 experiments. Keep it shorter since contrastive learning in NLP is less common}

- (Optional) Some experiments for final v/s intermediate representations
}












\iffalse

This work provides theoretical examples and end-to-end experiments that highlight the limitations of current theoretical analyses (and assumptions) and argue that a complete and realistic theoretical understanding of the success of contrastive learning requires another crucial ingredient: the inductive bias of the function class. 


In particular, we theoretically show that even in the extreme \emph{block identity regime}---where each example is disconnected in the augmentation distribution, rendering existing theory vacuous---minimizing the contrastive loss within a function class can still produce meaningful representations and transfer bounds. Motivated by this analysis, we present experiments which suggest that common contrastive pre-training setups are indeed close to this regime. Furthermore, we show that different modifications \highlight{(small perturbations)} to the \highlight{standard} augmentation distribution (including artificially enforcing the block identity regime) result in different training and transfer behavior, depending on the choice of function class (i.e. architecture).
\fi





\iffalse
\highlight{This is the basic new story:

Most theoretical analyses justify minimizing a contrastive loss $\Lcont$ as follows: under appropriate distributional assumptions, any minimizer $f^{*} \in \argmin_{f} \Lcont(f)$ is shown to do well on downstream tasks.
Some make this robust by considering representations that are $\epsilon$-optimal, i.e. $\Lcont(f) - \Lcont(f^{*}) \le \epsilon$, where the $\epsilon$ error is typically due to finite sample and optimization issues.
% So downstream performance of $f$ is upper bounded by some function of $\Lcont(f) - \Lcont(f^{*})$
In practice, the loss $\Lcont$ is minimized using $f$ from a function class $\gF$ and a particular algorithm (e.g. Adam). This raises a few questions: }

(Q1) Is standard training actually minimizing $\inf_{f} \Lcont(f)$? Do we even need to do so for contrastive learning to be beneficial?

(Q2) Can we show guarantees for $\argmin_{f\in\gF} \Lcont(f)$ instead even though $\min_{f\in\gF} \Lcont(f) \neq \min_{f} \Lcont(f)$? Can those guarantees be stronger for some $\gF$ compared to guarantees that ignore the function class?

(Q3) Do we {\bf need} the assumptions needed in the previous analyses for contrastive learning to succeed, i.e. sufficient overlap between augmentations of images from the same class compared to images from different classes.

(Q4) What are other inductive biases?

\highlight{
We present experiments and theory that highlight limitations/pitfalls of many earlier analyses of contrastive learning and open up a new dimension of understanding, namely, the inductive biases of the model architecture and training procedure.}


(Q1) Show experimental scenarios (\highlight{hash experiment}) where standard training is far from minimizing $\argmin_{f} \Lcont(f)$. Despite this, contrastive learning succeeds.

(Q2+Q3) Theoretical results (\highlight{linear representations}) that show different behaviors of different function classes. Minimizing $\argmin_{f\in\gF} \Lcont(f)$ can lead to much better (non-vacuous) guarantees compared to $\argmin_{f} \Lcont(f)$, including better robustness.
Examples showing that contrastive learning can be beneficial even without the strong augmentation overlapping assumptions.

(Q3) \highlight{Evidence for non-overlapping of augmentation distribution?}

(Q4) There exist representations with comparable contrastive loss to standard training, but terrible downstream performance (\highlight{label orthogonal experiment}). Thus changing function class and training procedure could potentially lead to failure. \todo{standard training but force $f$ to not be able to predict labels}. \highlight{Role of intermediate representation.}

================

Here's an example that succinctly demonstrates the point. Consider inputs that are vertices of the hypercube $\{\pm 1\}^{D}$, and downstream label is a linear classifier on the first $k\ll D$ coordinates. Augmentation $x'$ of $x$ is obtained by randomly sampling $\tau \in [0, 1]$ and downscaling $x[k:]$ by $\tau$, so $x'[:k] = x[:k]$ and $x'[k:] = \tau ~x[k:]$. (this can be generalized to only downscaling a random subset of $x[k:]$, analogous to randomly downscaling some aspect of an image like color or amount of blur)
Since the first $k$ coordinates are never affected while other coordinates are scaled down some time, it seems like contrastive learning should help. But it's easy to see that this is the "block identity" setting, since the original input $x$ can be recovered from an augmentation by doing $x = sign(x')$, so there exist minimizers of the contrastive loss that basically has 50\% performance on downstream.
However if the representation class is linear in $x$, then CL provably does well on downstream task. In fact in experiments, even an MLP representation does well on the downstream task. Both linear and MLP representations don't learn the optimal representation ever

% The following are the issues with this: firstly there is no guarantee that training in practice learns the minimizer or even something that is close to $\min_{f} \Lcont(f)$.
% If the representation comes from a class $\gF$, then one can only hope to learn $\argmin_{f\in\gF} \Lcont(f)$, and more practically something that is $\epsilon$-optimal w.r.t. to this.
% Why should we expect such representations to do well on downstream tasks? and can these guarantees be stronger when the representation function class $\gF$ is taken into account?



- Show theoretical (and empirical) scenarios where contrastive learning using a particular function class (ResNet) can learn a good representation without learning $\argmin_{f} \Lcont(f)$. In fact a different function class (MLP) that can make the contrastive loss much smaller and closer to $\argmin_{f\in\gF} \Lcont(f)$ does poorly on the downstream task. This highlights the importance of the function class bias

- Show experimental evidence that the training procedure also kind of matters

- Theoretical analysis for linear representation learning that can capture some of these phenomenon

- Point out other intriguing properties that are not yet captured by theory and open up an interesting set of practically relevant theoretical questions.



\todo{

- Fix the label orthogonal experiment by using predicted augmentation labels as opposed to original image label. Also try not deleting all directions, but only a few

- Run for multiple number of training samples to show that gap is small

- Any analysis for finite samples?

- Analysis for regularized objective

- Something about $f$ being better than $g$. May be some supervised learning experiment of fitting random labels

- Main pipeline for difference in theory and practice
\begin{itemize}
    \item Augmentation representation to image representation: taking average of augmentation representation is better
    \item $f \rightarrow g$ issue: theory deals with $g$, practice evaluates $f$. no theory to understand why this happens
    \item Comparing contrastive loss (CL) to absolute minimal CL: training might not even minimize CL, depending on the function class. This might actually be beneficial for us.
    \item Suboptimal solution analysis: finite samples based analysis doesn't exist.
\end{itemize}
}
% \begin{center}
\highlight{Separator}
% \end{center}



\ns{we identify the failure modes and formalize the extreme version of this failure through the non-overlapping augmentation setting.}

Thus, our work serves as a checkpoint and critique of current theoretical analyses and opens up a new dimension of understanding of contrastive learning. 



\ns{
New narrative: Overlap in augmentation distribution does not capture the full power of CL. In fact standard training may even yield absolute minimizer of CL, which is what earlier theories rely on. Yet it learns something meaningful. Will demonstrate this point through experiments and capture in simple theory.

Forcing training to be orthogonal to labels can still lead to reasonably small CL loss but terrible downstream performance.
So both function class and algorithm will be shown to matter.
Elements used: hash (replace entire pixels), hash with bit shift, training with fewer samples, label orthogonality, representation orthogonality.

- with hash pixels MLP can go to minimizer, while CNN does not. CNN trained appropriately can match those MLP reps, so it has to do with GD algorithm as well. So 

- with bit\_shift=0 neither CNN or MLP can go to minimizer. bit\_shift=7 MLP can go to minimizer, CNN cannot

- label orthogonal experiment: learn representation that makes CL loss small while enforcing orthogonality to labels. this can achieve low CL loss (5.45) but not as small as normal training (5.35), but terrible downstream performance ($\sim$ 30\%). Instead, comparing to standard CL training but with fewer (10k) samples insteads, min CL loss is 5.45 but downstream is $\sim$80\%.

- adding class wise diversity term can make CL okay-ish small, but terrible downstream performance

- forcing representation to not predict downstream can only get so much performance

- $f$ saves us in many places, even if $g$ is bad in some of the above cases.

- Issues with non-overlapping distribution: lower bound
}


\ns{New points
\begin{itemize}
    \item $f$ can be significantly better than $g$ for weird losses
    \item avg. of augmentation rep is better than image rep
    \item $\exp$ of ips is better than ips for spectral loss
    \item 
\end{itemize}
}

% We hope that the theoretical examples and underlying intuitions behind them will help future research on better understanding contrastive learning and related methods.
% As a starting point, using current state-of-the-art contrastive learning pipelines, we give empirical evidence for the affect of the choice of function class used for the representation on the downstream performance of the learned representation, even when the performance on the contrastive objective is identical. This highlights the need to account for function class in the transfer bounds. 

% \ns{evidence that function class }
% present diagnostic experiments that cast doubts on the validity of the assumption 
% \ns{Motivate non-overlapping setting }


% Through experiments, we first  representations obtained from minimizing contrastive loss can have drastically different downstream performance depending on the choice of underlying function class used for the representation even when the contrastive loss is the same. Furthermore, we argue that  

% Motivated by diagnostic experiments on large-scale setups, we highlight simple settings where the performance of contrastive loss-minimizing representations depends strongly on the underlying function class. Furthermore, we argue that theory fail to contain downstream class information-- we show that theory that neglects to restrict the function class produces vacuous transfer guarantees. \cz{Finish experiment summary when more stuff is in.}


% \paragraph{Summary of contributions.} Through varied theoretical examples, we show that the success or failure of contrastive learning can depend on interactions between the inductive bias of the function class. In particular, we point out that in the \emph{block identity regime}---where each example is disconnected in the augmentation distribution, rendering existing theory vacuous---minimizing the contrastive loss within a function class can still produce meaningful representations and transfer bounds. Motivated by this analysis, we present experiments which suggest that common contrastive pretraining setups are indeed close to this regime. We show that different modifications to the augmentation distribution (including artificially enforcing the block identity regime) results in different training and transfer behavior, depending on the choice of function class (i.e. architecture).

% This work provides an alternative perspective on why contrastive learning with augmentations works, and makes initial progress on understanding the complex interactions between augmentations and the function class.


% \ns{Diagnostics, formalizer, rebuttal (limitations of formalization), solutions}

% \begin{itemize}
%     \item[Diagnostic:] Capturing the idea (that is missing in previous analyses) that how well a representation, that does reasonably well on the contrastive task, will end up doing well on a downstream task can depend on the representation function class (and potentially also the training algorithm).
%     \ns{Link to MLP vs resnet vs permuted  figure to explain what inductive bias means in this context.}

%     \item \ns{This is a bit over-the-top for now, can mellow down appropriately later.} The current analyses rely strongly on the overlap between augmentation distribution, i.e. different inputs (especially those that belong to the same class), have a non-trivial overlap in the distribution of augmentations that they each produce.
%     We argue, through experiments and theoretical examples, that this assumption may not be true, and in fact there might very little to no overlap between the augmentation distributions which will lend the existing bounds vacuous \ns{link to augmentation classification experiment figure}.
%     In this work we show that not just the priori analyses, but any analysis that is function class independent (that ignores function class bias) will lead to a vacuous bound in the worst case of non-overlapping augmentation distributions.
%     On the other hand, we demonstrate through theoretical results and examples that show how incorporating the ``inductive bias'' of the function class in the analysis can get around this and can lead to meaningful non-vacuous bounds even in the non-overlapping augmentations case.

%     \item Highlight that this paper is not meant to be a complete theory that fully explains the success of contrastive learning.
%     It serves as a checkpoint and critique of current theoretical analyses and opens up a new dimension of understanding of contrastive learning.
%     We hope that the theoretical examples and underlying intuitions behind them will help future research on better understanding contrastive learning and related methods.

% \end{itemize}

% \ns{Something about how this connects to many existing intuitions about contrastive learning. InfoMax, InfoMin, transfer bounds, information theoretic benefits, instance discrimination}


\subsection{Main components}
\begin{itemize}[leftmargin=*]
    \item (Experiment) Different transfer bound for different function classes (almost done), \Cref{fig:arch_diff}.
    \item (Experiment) Evidence for non-overlapping setting. Augmentation classification experiment: given an augmentation, learn a model to identify the original image it came from.
    \begin{itemize}
        \item Currently gets ~99\% on 5000-way classification task for images from a CIFAR-10 class. Hope that this number is already surprising enough.
        \item Try ResNet-50, might do better
        \item Look at the confusion matrix, which images are confused with each other. Can images be clustered into some 100 clusters for which the cluster identification (instead of image identification) accuracy is much higher?
        \item Learn classifier in a way that can generalize to test images. Some meta-learning framework?
        \item Use representation to separate test images
        \item Use representations to get small contrastive loss
        \item CIFAR-100 might be easier, but less impressive
        \item (Extra) Evaluate representations on downstream, surprising if it still does well (how to combine different classes?)
        \item (Extra) Class 1 reps for class 2 classification
    \end{itemize}
    \item (Experiment) MD5 experiment (basically done). Replace 16 random pixels of an augmentation with MD5 hash of the original image generating it.
    This ensures that augmentation distributions are non-overlapping.
    \begin{itemize}
        \item MLP gets lower contrastive loss (both SimCLR and spectral) than ResNet-18, but gets much worse downstream accuracy (~20\% v/s ~90\%). So MLP can presumably pick up on the 16 pixels while CNN cannot (does not)
    \end{itemize}
    \item (Experiment) ``Sweet spot'' experiment. Try different augmentations (e.g. scale of random cropping) for different architectures
    \begin{itemize}
        \item The ``sweet spot'' (best augmentation) was the same for MLP and ResNet-18
        \item (Extra) Can sweet spot be predicted without labels (e.g. time to fit random labels)
    \end{itemize}
    \item (Theory) Connect augmentation classification error to eigen-gap. Small augmentation classification error means small eigengap (and large tranfer bound). Showed in \Cref{lem:bayes_error_eigen_gap}.
    \item (Theory) Low-rank linear representation (given a original feature map $\phi$); $f(x) = W \phi(x)$, where $W$ is learnt.
    Transfer bound depends on eigenvalues of augmentation averaged features of $\phi$ (\Cref{thm:low_rank_result}).
    With a full rank $\phi$ one can pretty much recover the result from \citet{haochen2021provable}.
    \begin{itemize}
        \item Give an interpretation to main result
        \item Topic modeling example with $\phi$ being bag-of-bigram representation, and augmentation is replacing p\% random tokens with random words.
        The eigengap is exponentially small in $N$ (document length), but the gap is constant gap if the linear representation result is used.
        \item Hypercube example, where $\phi$ is identity map, label depends only on a subset $S$ of coordinates, augmentation is scaling down a random subset of coordinates disjoint with $S$ by factor $\tau \ll 1$
        \item \ns{Ignore} Convert a kernel into a low rank representation by looking at projection onto finite number of independent datapoints. Can fewer samples be ever better? Related to some NTK experiment
    \end{itemize}
    \item (Theory) Norm-bounded linear represetation, $f(x) = W \phi(x)$ with $\|W\|_{F}^{2} \le B$.
    \begin{itemize}
        \item Result currently has a lot of assumptions, (a) block identity, (b) spectral separability, (c) a specific value of $B$. Relaxing 1 or more of these would help. In thw worst case we can phrase the result differently: guarantees for a non-low rank function class even in the bad case of non-overlapping distributions.
        \item Figure out a good example
    \end{itemize}
    \item (Theory) Theoretical argument for non-overlapping (block-identity) being bad.
    No contrastive like objective can learn anything meaningful.
    \item *** Connect theory to practice!
    \item (Misc experiment) Try bag-of-bigrams experiments with random word replacement for text classification dataset like SST, AG News \ns{?}.
    % \item (theory) reverse result: if $k^{\text{th}}$ eigenvalue is lower bounded, then the classification error is lower bounded too. The eigen-gap can be upper bounded as $\lambda_{k+1} - \lambda_{k} \le \lambda_{k+1} \le \frac{\bar{\rho} ~\text{Bayes-error}(\gA)}{1 - \nicefrac{k}{|\Xorig|}}$, where $\bar{\rho} = \frac{\gDbar_{\max}}{\gDbar_{\min}}$ is the ratio of max and min probabilities over inputs.
\end{itemize}


\fi

==> table_fig/md5_table.tex <==
\begin{table}[t!]
\begin{center}
	\caption{Performance of ResNet, ResNet-Perm and MLP architectures on augmentations that have the MD5 hash of the image generating it encoded in 16 fixed pixels, leading to a non-overlapping augmentation setting. While the MLP does very well on the validation contrastive loss, the downstream performance on CIFAR-10 is much lower. This suggests that whether or not the non-overlapping augmentation setting can lead to useful representation can depend strongly on the function class used to learn the representation.}
	\label{table:hash}
\begin{tabular}{ |c|c c|c c| } 
% \begin{tabular}{ |c|c|c|c|c| } 
 \hline
    &  \multicolumn{2}{c}{SimCLR} & \multicolumn{2}{c}{Spectral} \\
    &  $\Lcont$    & $\Lclf$   & $\Lspec$  & $\Lclf$\\
 \hline
 ResNet &  \ns{5.36}   &      &   \ns{-1.70}    &  \\
 ResNet-Perm &     &      &       & \\
 MLP &  \ns{4.92}   &      &    \ns{-1.99}   & \\
 \hline
\end{tabular}
\end{center}
\end{table}

==> table_fig/nlp_scatter_plot.tex <==
\begin{figure}
    \centering
        \includegraphics[width=.9\linewidth]{media/cifar-2x2.pdf}
        \vspace{-0.1in}
    \caption{Contrastive loss $\rightarrow$ accuracy transfer plots for Wiki-3029 and AG News with different architectures and augmentations. \todo{These are placeholder plots, replace with correct NLP plots.}}%{\bf TL:} Full pipeline of augmentations from SimCLR \citep{chen2019simple} (described in \Cref{sec:vision_exp}). {\bf TR:} Remove random cropping. {\bf BL:} Remove random cropping and horizontal flip. {\bf BR:} Add hash pixels to the image as described in \Cref{sec:vision_hash_exp} to make it a non-overlapping setting. Here we observe transfer collapse happen for ViT, despite ResNet-18 working totally fine.}
    \label{fig:nlp_scatter_plot}
\end{figure}

==> table_fig/transfer_fig.tex <==
\begin{figure*}[ht!]
    \centering
    % \hspace{-0.8cm}
    \includegraphics[trim={0, 20.5cm, 3, 0cm}, clip, scale=0.5]{./media/nceLoss.pdf}
    \caption{Downstream test accuracy as a function of validation NCE loss for both a standard ResNet and a ResNet that's been trained on data with randomly permuted pixels. Here we toggle two experimental variations. In one, we perform downstream classification using either the representation obtained from the projection head (which is closer to what our theory describes), or the representation obtained before the projection head (which is what is typically done in practice). We also vary the number of augmentations done, using either all five done in standard NCE training or only three, which excludes both random crops and horizontal flips. Regardless, all experiments show that the standard ResNet outperforms the permuted ResNet on downstream classification, even when both models obtain similar NCE loss.}
    \label{fig:arch_diff}
\end{figure*}

==> table_fig/wiki_scatter_plot.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[scale=0.25]{media/plot_drop_top_10_accuracy.pdf}
     \includegraphics[scale=0.25]{media/plot_drop_permute_top_10_accuracy.pdf}
     \vspace{-0.1in}
    \caption{Top-10 test classification accuracy against contrastive validation loss on Wiki3029 for various augmentations and models.}
    \label{fig:text_experiments}
     \vspace{-0.1in}
\end{figure}

==> theory_backup.tex <==
% !TEX root = main.tex

\section{Theory}


\begin{enumerate}
    \item Low rank linear representation result. Kind of straightforward, because gap will only depend on the subspace.
    \item Norm bounded linear representation, with non-overlapping augmentation graph. Kind of straightforward, because gap will only depend on the subspace
    \item Examples: topic modeling, boolean hypercube (?), Gaussian (?)
\end{enumerate}

Hoping to incoporate function class in transfer bound, beyond just a generalization bound.
Simplest setup, $\Xorig$ is the set of original images, $\Xaug$ is set of augmentations. $\A\in\R^{|\Xaug|\times|\Xaug|}$ is the augmentation distribution/graph.
Goal of spectral contrastive learning is to learn representation $f:\Xaug\rightarrow\R^k$.
Let $F\in\R^{|\Xaug|\times k}$ denote the matrix version of $f$, where the row $F_x = f(x)$.
The contrastive loss is defined as
\begin{align}
    \Lspec(f) 
    &= -2\ex_{(x,x^{+})} f(x)^{\top} f(x^{+}) + \ex_{x,x^{-}} \left(f(x)^{\top} f(x^{-})\right)
    \label{old_eqn:contrastive_loss}\\
    &= \|D^{-\half}\A D^{-\half} - D^{\half}FF^{\top} D^{\half}\|_F^2 - \|D^{-\half}\A D^{-\half}\|_F^2\nonumber
\end{align}
where $D\in\R^{|\Xaug|\times |\Xaug|}$ is the diagonal matrix with the marginal probabilities of augmentations.
The representation $f$ typically comes from a function class $\gF$.

Prior analysis show transfer bound by following the recipe
\begin{itemize}
    \item Show that for $f^{\star}\in\argmin_{f} \Lspec(f)$, $\Lclf(f^{\star}) \le \alpha_{\text{apx}}$
    \item For $f$ such that $\Lspec(f) \le \Lspec(f^{\star}) + \epsilon$, we have $\Lclf(f) \le \Lclf(f^{\star}) + \frac{\epsilon}{\trf_{\text{trf}}}$
\end{itemize}
For these bounds, both coefficients $\alpha_{\text{apx}}$ and $\trf_{\text{trf}}$ depend only on the distribution $\gD$ and grouth truth labels $y(\cdot)$.

For Spectral-paper (HaoChen et al.) \todo{add citation}:

\[\alpha_{\text{apx}} = \frac{\alpha}{\lambda_k} \qquad \trf_{\text{trf}} = \lambda_k - \lambda_{k+1}\]


We want to show bounds where both $\alpha$ and $\trf$ can depend on the function class $\gF$, and can potentially lead to much better (non-vacuous) bounds.







\subsection{General class (trivial bound)}

Recall that the contrastive loss is
\begin{align*}
    \Lspec(f) = -2\ex_{(x,x^{+})} [f(x)^{\top} f(x^{+})] + \ex_{x,x^{-}} \left[\left(f(x)^{\top} f(x^{-})\right)^{2}\right]
\end{align*}
A function class $\gF\subseteq\{f:\Xaug\rightarrow\R^k\}$ of representations can be considered.
% \highlight{A special case is: $\gF = \gF_{1}^{\times k} \subseteq \{f:\Xaug\rightarrow\R^k\}$ where $\gF_1\subseteq\{f:\Xaug\rightarrow\R\}$ is the scalar function.}
% \ns{Incomplete}
For a matrix $F\in\R^{|\Xaug|\times k}$, we define the contrastive loss $\Lspec(F)$ as the loss for the representation function $f$ where $f(x) = F_x$.

Let $g^{\star}\in\R^{\Xorig}$ be the vector of ground truth predictor, i.e. $g^{\star}_{\bar{x}} = \frac{1}{|\Xorig|} y(\bar{x})$ (consider binary classification for now).
The joint distribution can be factorized as $\A  = \Abar^{\top}\bar{D}\Abar\in\R^{\Xaug\times\Xaug}$, where rows of $\Abar\in\R^{\Xorig\times\Xaug}$ are the conditional distribution of $P(x\mid\bar{x})$ and $\bar{D}$ is the diagonal matrix of marginal probabilities of $\Xorig$.
We define the classification loss on original images $\Xorig$ as
\begin{align}
    \Lclf(f) = \Lclf(F)
    = \inf_{w\in\R^{k}} \ex_{\bar{x}} \left(\ex_{x\mid\bar{x}}[f(x)|\bar{x}]^{\top} w - y(\bar{x})\right)^2
    = \inf_{w\in\R^{k}} \left\|\bar{D}^{-\half}\Abar Fw - g^{\star}\right\|^2
    \label{old_eqn:clf_loss}
\end{align}
We are interested in the following quantity that characterizes the amount of transfer
\begin{align}
    \trf_{\gF}(\beta) 
    &= \inf_{\substack{\Lclf(f) \ge \beta\\f\in\gF}} \Lspec(f) - \inf_{\substack{f\in\gF}} \Lspec(f)
    % \trf_{\gF}(\beta) 
    % &= \inf_{\substack{\|P_{F}^{\perp} g^{\star}\|^2 \ge \beta\\F\in\gF}} \Lspec(F) - \inf_{\substack{F\in\gF}} \Lspec(F)
    \label{old_eqn:trf_def}
\end{align}
This quantity will (trivially) give the following transfer bound
\begin{fact}
\label{old_fact:transfer}
    Any $f\in\gF$ that satisfies $\Lspec(f) - \inf_{f^{\star}\in\gF} \Lspec(f^{\star}) \le \epsilon$ will suffer a transfer error of $\Lclf(f) \le \trf_{\gF}^{-1}(\epsilon)$, whenever the inverse exists. \ns{Handle non-invertible $\trf$} 
\end{fact}






\subsection{Linear representation}
For fixed representations $\Phi\in\R^{|\Xaug|\times D}$, we consider the function class \begin{align*}
    \gF_{\Phi} = \{F = F_0 + \Phi W \mid W\in\R^{D\times d}\}
\end{align*}
We further consider a restricted function class
\begin{align*}
    \gF_{\Phi,B} = \{F = F_0 + \Phi W \mid W\in\R^{D\times d}, \|W\|^2_F \le B\}
\end{align*}
The {\em inductive bias} of algorithm like gradient descent is being abstracted away as Frobenius norm bound. It is not clear if this is correct.
Instead we can just consider an algorithm that finds the minimizer of the following regularized loss
\begin{align*}
    Alg_{\Phi, \tau}
    &= \Phi \left( \argmin_{W\in\R^{D\times d}} \left\{ \Lspec(\Phi W) + \tau \|W\|_F^2 \right\}\right)
    = \argmin_{F} \left\{ \Lspec(F) + \tau \|F\|_{(\Phi\Phi^{\top})^{-1}} \right\}\\
    &= \argmin_{F} \left\{ \Lspec(F) + \tau~ \tr\left(F^{\top} (\Phi\Phi^{\top})^{-1} F\right) \right\}
\end{align*}

\paragraph{Gradient descent (do not know how to analyze):}
The most ambitious goal is to analyze gradient descent itself
\begin{align*}
    W_{t+1} = W_{t} - \eta \nabla_{W} \Lspec(\Phi W_{t})
\end{align*}
Here is why this problem is difficult. Even for $\A =I_{|\Xaug|}$ it is not clear how to characterize the solution found by gradient descent when there are multiple minimizers.
Let $\Phi = USV^{\top}$ be the SVD, then the dynamics of gradient descent can be written as
\begin{align*}
    \nabla_{W}
    &= - \Phi^{\top} (\A  - \Phi W W^{\top} \Phi^{\top}) \Phi W
    = - \Phi^{\top} \A  \Phi W - \Phi^{\top}\Phi W W^{\top} \Phi^{\top} \Phi W\\
    &= - V S U^{\top} \A  U S V^{\top} W - V S^2 V^{\top} W W^{\top} V S^2 V^{\top} W\\
    V^{\top} \nabla_{W}
    &= -S U^{\top} \A  U S (V^{\top} W) - S^2 (V^{\top} W) (V^{\top} W)^{\top} S^2 (V^{\top} W)
\end{align*}
Let $\tilde{W} = V^{\top} W \in \R^{D \times d}$, then 
\begin{align*}
    \tilde{W}_{t+1} = \tilde{W}_{t} + \eta \left( S U^{\top} \A  U S - S^2 \tilde{W}_{t} \tilde{W}_{t}^{\top} S^2 \right) \tilde{W}_{t}
\end{align*}
If $\A  = I$ the dynamics reduces to
\begin{align}
    \tilde{W}_{t+1} = \left( I + \eta S^2 - \eta S^2 \tilde{W}_{t} \tilde{W}_{t}^{\top} S^2 \right) \tilde{W}_{t}
\end{align}
It looks like some power method type of method, but not exactly.
Analyzing this case would be interesting.
Note that $S$ is the diagonal matrix of singular values of $\Phi$.




\iffalse
\subsubsection{Simple example 1}

Recall that $\Xorig$ is the set of {\em original images} and $\Xaug$ is the set of all augmentations of all images.

% \sg{Confusion between $\Xaug$ and $\Xorig$ above and below. I would suggest using $\Xaug$ and $\gX_{\text{aug}}$}.
% \ns{Makes sense, changed}

For this example assume that $\Xorig$ and $\Xaug$ are finite.
\paragraph{Augmentation distribution $\A $:}
$\A \in\R^{\Xaug\times\Xaug}$ is block diagonal with $|\Xorig|$ blocks, with each non-zero entry being $\frac{|\Xorig|}{|\Xaug|^2}$. $D = \frac{1}{|\Xaug|}~I_{|\Xaug|}$ is the diagonal matrix of uniform marginal distribution; $\An = D^{-\half} \A  D^{-\half}$. 
In this case, $\trf_{\text{trf}} = 0$, so previous bounds are vacuous when suboptimality $\epsilon > 0$.
This makes the contrastive loss equal to
\begin{align}
    \Lspec(F)
    &= \left\|\An - D^{\half} FF^{\top} D^{\half}\right\|^2 = \left\|\An - \frac{1}{|\Xaug|} FF^{\top}\right\|^2
    \label{old_eqn:contrastive_eg_1}
\end{align}

\paragraph{Function class $\gF$:}
Let $g^{\star}\in\R^{\Xaug}$ be the ground truth labels on the augmentations such that $g^{\star}_{x} = \frac{1}{|\Xaug|} y(x)$, where $y(x)\in\{\pm 1\}$ is the ground truth binary label. Note that $\|g^{\star}\| = 1$.
We consider the fixed linear representation $\Phi$ through the kernel $K=\Phi\Phi^{\top}\in\R^{\Xaug\times \Xaug}$ parametrized by $G>1$
\begin{align}
    % K &= (G-1) g^{\star} {g^{\star}}^{\top} + I_{|\Xaug|}\\
    K &= (G-1) g^{\star} {g^{\star}}^{\top} + \A  + P^{\perp}_{\A }
    % K(\epsilon_1, \epsilon_2, \epsilon_3) = \epsilon_{1} \frac{1}{|\Xaug|} g^{\star}{g^{\star}}^{\top} + \epsilon_{2} \frac{1}{|\Xaug|} \A  + \epsilon_{3} \left(I_{|\Xaug|} - \frac{1}{|\Xaug|} \A \right)
\end{align}
In this setup, $G$ is going to be quite large, roughly of the order of $\frac{|\Xaug|}{|\Xorig|}$. This is because you are competing against the second term that has trace of $|\Xaug|$.
The function class then is defined as 
\begin{align}
    \gF_{B}
    &= \{F\in\R^{\Xaug\times d} \mid F = \Phi W, ~\|W\|_F^2 \le B\}\\
    &= \{F\in\R^{\Xaug\times d} \mid \|F\|^{2}_{K^{-1}} = \tr(F^{\top} K^{-1} F) \le B\}
\end{align}

\paragraph{Transfer bound:} For this augmentation graph $\A $ and function class $\gF_{B}$, we will show how different values of $B$ affects the transfer bound by showing a lower bound on $\trf_{\gF}(\beta)$ from \Cref{eqn:trf_def} and then invoke \Cref{fact:transfer}.
\begin{prop}
\label{old_prop:simple_eg_1}
    (Upper bound) Let $\bar{B} = \frac{B}{|\Xaug|}$. If $\bar{B} < k-1$, then we have the following for small constants $1 \le c_1,c_2 \le 10$
    \begin{align*}
        % \trf_{\gF_{B}}(\beta) &\gtrsim \frac{(k-\bar{B})}{c_1 k}\beta - \frac{c_2}{G}
        \trf_{\gF_{B}}(\beta) &\gtrsim \left(1-\frac{1}{G}\right)^2 \frac{(k-\bar{B})}{k}\beta
    \end{align*}
    So for any representation $f\in\gF_{B}$ that is $\epsilon$-optimal, i.e.$\Lspec(f) - \inf_{f^{\star}\in\gF_{B}} \Lspec(f^{\star}) \le \epsilon$, \Cref{fact:transfer} gives us
    \begin{align*}
        \Lclf(f)
        % &\lesssim \frac{c_1 k}{(k-\bar{B})} \left(\epsilon + \frac{c_2}{G}\right)
        &\lesssim \left(1-\frac{1}{G}\right)^{-2}\frac{k\epsilon}{(k-\bar{B})}
    \end{align*}

    (Lower bound) On the other hand if $\bar{B} \ge k$, we have $\trf_{\gF_{B}}(\beta) = 0$ for every $\beta\in[0,1]$, which gives a vacuous transfer bound.
\end{prop}
The above result suggests that a small enough function class w.r.t. a natural norm can have a much better transfer bound.
Roughly, smaller $B$ (smaller function class) and larger $G$ (more bias of function class towards ground truth labels) lead to a better transfer error.
{\bf $G$ will roughly be of the order of $\frac{|\Xaug|}{|\Xorig|}$, i.e. number of augmentations per image. So this kind of weakly justifies use of multiple augmentations.}

\ns{What is the point of this bound? Why is the kernel norm relevant? It is trivial to construct another function class if we restrict ourselves to norms, for e.g. if $\gF$ only contains $g^{\star}{g^{\star}}^{\top}$. So definitely some justification is needed for this norm based construction.}

\ns{In this case, not all small values of $B$ can get minimum contrastive loss. Might be important to have such a function class instead? Adding linear layer on top of reps can help with this?}


\begin{proof}[Proof sketch for \Cref{prop:simple_eg_1}]
    The definition of $\trf_{\gF_{B}}(\beta)$ from \Cref{eqn:trf_def} is restated below
    \begin{align*}
        \trf_{\gF}(\beta)
        &= \kappa(\beta) - \kappa(0)\text{, where}\\
        \kappa(\beta)
        &= \inf_{\substack{\Lclf(f) \ge \beta\\f\in\gF}} \Lspec(f)
    \end{align*}
    Note that again we use $f:\Xaug\rightarrow\R^k$ and $F\in\R^{\Xaug\times k}$ interchangeably.
    Let $\frac{1}{|\Xaug|}FF^{\top} = \sum_{i=1}^{k} \sigma_i \brf_{i} \brf_{i}^{\top}$ be the eigendecomposition, then
    \begin{align}
        \brf_i\in\R^{\Xaug}, |\brf_{i}|=1, \brf_i^{\top} \brf_j = 0\text{, if }i\neq j
    \end{align}
    For $X\in\R^{n\times m}$, let $P_{X} = XX^{\dagger}\in\R^{n\times n}$ be the projection matrix for column space of $X$.
    % Since all eigenvalues of $\An$ are 1, we can decompose it as $\A $ 

    {\bf Step 1:} Notice that for any $F$, $\Lspec(P_{\A }F) \le \Lspec(F)$, $\|P_{\A }F\|_{K^{-1}} \le \|F\|_{K^{-1}}$ and $\Lclf(P_{\A }F) = \Lclf(F)$.
    So we can only consider functions $f$ that are augmentation invariant, i.e. $P_{\A }F = F$, since it only makes the contrastive loss and the norm small.
    \begin{align}
        P_{\A }F = F, \text{ so } \A \brf_i = \brf_i
    \end{align}
    \ns{The $\Lclf(P_{\A }F) = \Lclf(F)$ bit is not true for another $\A $. Need the ground truth label to be an eigenvector of $\A $ with eigenvalue 1, which may be strong and unrealistic.
    There might be augmentation variant parts of $K$ that might better predict $g^{\star}$ rather than enforcing augmentation invariant.
    }

    % 
    {\bf Step 2:} Show that $\Lclf(f) = 1 - \|P_{F} g^{\star}\|^2$, where $P_{F} = FF^{\dagger} = \sum_{i=1}^{k} \brf_i\brf_i^{\top}$.
    So the condition $\Lclf(f) \ge \beta$ can be replaced by
    \begin{align}
        \|P_{F} g^{\star}\|^2 = \sum_{i=1}^{k} \left(\brf_{i}^{\top} g^{\star}\right)^2 \le 1 - \beta
    \end{align}
    %
    {\bf Step 3:} Since $K = (G-1) g^{\star}{g^{\star}}^{\top} + I$, $K^{- 1} = I - \frac{G-1}{G}g^{\star}{g^{\star}}^{\top}$. Thus the norm constraint of $\|F\|^2_{K^{-1}} = \tr\left(F^{\top} K^{-1} F\right) \le B$ can be replaced by
    \begin{align}
        |\Xaug| \sum_{i=1}^{k} \sigma_i \brf_i^{\top} K^{-1} \brf_i
        &\le B\nonumber\\
        \sum_{i=1}^{k} \sigma_i \left(1 - \frac{G-1}{G}(\brf_i^{\top}g^{\star})^2\right)
        &\le \frac{B}{|\Xaug|} = \bar{B}
    \end{align}
    %
    {\color{purple} {\bf Step 3 (error):} Suppose we only know that $K$ has square loss with respect to the best linear predictor bounded by $\Delta$. This implies ${g^{\star}}^{\top} K^{-1} g^{\star} \le \Delta$.  Thus the norm constraint of $\|F\|^2_{K^{-1}} = \tr\left(F^{\top} K^{-1} F\right) \le B$ can be relaxed to
    \begin{align}
        &|\Xaug| \sum_{i=1}^{k} \sigma_i \brf_i^{\top} K^{-1} \brf_i
        \nonumber\\
        &=|\Xaug|\sum_{i=1}^{k} \sigma_i \left((\brf_i^{\top}g^{\star})^2 {g^{\star}}^{\top} K^{-1} g^{\star} + \left(1 - (\brf_i^{\top} g^{\star})^2\right) {\brf_{\perp, i}}^{\top} K^{-1} {\brf_{\perp, i}}\right) \nonumber\\
        &\le |\Xaug|\sum_{i=1}^{k} \sigma_i \left((\brf_i^{\top}g^{\star})^2 \Delta + \left(1 - (\brf_i^{\top} g^{\star})^2\right) \lambda_{\min}(K)\right) \nonumber\\
        &= |\Xaug|\lambda_{\min}(K)\sum_{i=1}^{k} \sigma_i \left(1 - \left(1 - \frac{\Delta}{\lambda_{\min}(K)}\right)(\brf_i^{\top}g^{\star})^2\right) \le B
    \end{align}
    Here $G = \lambda_{\min}/\Delta$, we could assume $\lambda_{\min}(K)$ to be a constant.
    }
    \ns{I think we need to replace it with a weaker condition rather than stronger condition}
    
    {\bf Step 4:} Since $F$ is invariant to augmentations (from Step 1), the contrastive loss can be written as
    \begin{align}
        \Lspec(F) = \sum_{i=1}^{k} (1 - \sigma_i)^2
    \end{align}
    %
    {\bf Rephrase the problem:} Let $\bm{\sigma} = (\sigma_1, \cdots, \sigma_k)$ and $\bm{\mu} = \frac{1}{1-\beta}\left((\brf_1^{\top}g^{\star})^2, \dots, (\brf_k^{\top}g^{\star})^2\right)$.
    If $k$ is not too large, then $\bm{\mu}$ can be learn freely s.t. $\bm{\mu}\in[0,\frac{1}{1-\beta}]^k$ despite the conditions $\|\brf_i\| = 1$ and $\brf_i^{\top}\brf_j = 0$.
    All of this can be reduced to
    \begin{align*}
        \kappa(\beta)
        &= \inf_{\bm{\sigma},\bm{\mu}} \|\bm{1} - \bm{\sigma}\|^2\\
        \text{s.t. } \bm{\sigma}&\ge 0, \bm{\mu}\in[0,1]^k\\
        \bm{1}^{\top}\bm{\mu} &\le 1-\beta\\
        \bm{\sigma}^{\top} \left(\bm{1} - \frac{G-1}{G} \bm{\mu}\right) &\le \bar{B}
    \end{align*}
    \ns{The choosing freely bit may not be true for general $K$}
    %

    {\bf Solving for $\kappa(\beta)$:} In this case we can pretty much find a closed form expression.
    We do so by first solving the minimization problem for a fixed $\bm{\mu}$.
    Let $\rho_{\bm{\mu}} = \bm{1} - \frac{G-1}{G} \bm{\mu}$
    \begin{align*}
        \kappa_{\bm{\mu}}(\beta)
        &= \inf_{\bm{\sigma}} \|\bm{1} - \bm{\sigma}\|^2\\
        \text{s.t. } \bm{\sigma}&\ge 0,~
        \bm{\sigma}^{\top} \rho_{\bm{\mu}} \le \bar{B}
    \end{align*}
    The minimizer $\bm{\sigma^{\star}}$ of the above problem is simple to obtain through Langrangian dual, and is 
    \begin{align}
        \bm{1}-\bm{\sigma^{\star}} = \frac{\left(\bm{1}^{\top}\rho_{\bm{\mu}} - \bar{B}\right)_{+}}{\|\rho_{\bm{\mu}}\|^2}\rho_{\bm{\mu}}
    \end{align}
    This gives us the expression for $\kappa_{\bm{\mu}}(\beta)$
    \begin{align}
        \kappa_{\bm{\mu}}(\beta) = \frac{\left(\bm{1}^{\top}\rho_{\bm{\mu}} - \bar{B}\right)_{+}^2}{\|\rho_{\bm{\mu}}\|^2}
    \end{align}
    Using this expression, we can compute $\kappa(\beta)$
    \begin{align}
        \kappa(\beta) = \inf_{\substack{\bm{\mu}\ge\bm{0},\\\bm{1}^{\top}\bm{\mu}\le 1-\beta}} \kappa_{\bm{\mu}}(\beta)
    \end{align}
    With some algebraic manipulations, the best $\bm{\mu^{\star}}$ can be shown to be $\bm{\mu^{\star}} = (1-\beta) \bm{e}_{1}$.
    Plugging this into the above equation gives
    \begin{align}
        \kappa(\beta)
        &= \frac{\left(\bm{1}^{\top}\rho_{\bm{\mu^{\star}}} - \bar{B}\right)_{+}^2}{\|\rho_{\bm{\mu^{\star}}}\|^2}
        = \frac{\left(k - \frac{G-1}{G}(1-\beta) - \bar{B}\right)_{+}^2}{k-1 + \left(1 - \frac{G-1}{G}(1-\beta)\right)^2}
    \end{align}
    Firstly, it is easy to show that if $\bar{B} \ge k$, then $\kappa_{\bm{\mu}}(\beta) = 0$ since $(k-\frac{G-1}{G}(1-\beta) - \bar{B})_{+} = 0$.
    This is because $\bm{\sigma}$ is essentially allowed to sum up to $\bar{B}\ge k$, and so $\sigma_i$ can be set to 1 for every $i$ to make $\bm{1} - \bm{\sigma}=0$, thus proving the lower bound part of the proposition.

    For the other case, some more algebraic manipulations will lead to the result.
    It is simpler to look at the limit of $G\rightarrow\infty$.
    Here, the expression reduces to
    \begin{align}
        \kappa(\beta) = \frac{(k-\bar{B}-1 + \beta)^2}{k-1 + \beta^2}
    \end{align}
    Some algebraic manipulations reveal that $\kappa(\beta) - \kappa(0) \ge \frac{k-\bar{B}}{k}\beta$ when $\bar{B}<k-1$.
    For the case of finite $G$, additional additive error of $\gO\left(\frac{1}{G}\right)$ and multiplicative term of $\gO\left(1+\frac{1}{G}\right)$ will be incurred.
    Plugging this into $\trf_{\gF}(\beta) = \kappa(\beta) - \kappa(0)$ completes the proof.
    % \begin{align}
    %     \kappa(\beta) - \kappa(0) = 
    % \end{align}
\end{proof}
\fi




\subsubsection{Example 2 (Norm Bounded Case)}

\paragraph{Augmentations:}
\dipendra{Super minor: we should not refer to input as image. Let's be general.}
We will introduce some more notation that is going to be important for the more general results.
The augmentation graph/matrix $\A \in\R^{\Xaug\times\Xaug}$ is defined as
\begin{align}
    \A (x,x') = P_{aug}(x,x') = \ex_{\bar{x}}\left[P_{aug}(x \mid \bar{x}) P_{aug}(x' \mid \bar{x})\right]
\end{align}
Let $D\in\R^{\Xaug\times\Xaug}$ is the diagonal matrix with marginal probabilities $D(x,x) = P(x)$; easy to see that $\text{diag}(D) = \A \bm{1}$.
We also define the normalized augmentation graph as follows
\begin{align}
    \An = D^{-\half} \A  D^{-\half}.
\end{align}
We introduce the original image to augmentation {\em graph} matrix $\Abar\in\R^{\Xorig\times\Xaug}$ as the joint distribution of original images and augmentations, and its corresponding normalized version $\Abarn$.
\begin{align}
    \Abar(\bar{x},x)
    &= P(x, \bar{x}) = P(\bar{x}) P_{aug}(x \mid \bar{x})\\
    \Abarn
    &= \bar{D}^{-\half} \Abar D^{-\half}
\end{align}
where $\bar{D}\in\R^{\Xorig\times\Xorig}$ is the diagonal matrix of image marginal probabilities with $\bar{D}(\bar{x}) = P(\bar{x})$.
Given the sampling process of augmentations, it is not hard to see the following relations,
\begin{align}
    \A
    &= \Abar^{\top} \bar{D}^{-1} \Abar\\
    \An
    &= D^{-\half} \Abar^{\top} \bar{D}^{-1} \Abar D^{-\half}
    = \Abarn^{\top} \Abarn
    % & \dipendra{\mbox{I think you get $\Abarn^\top D^{\half} \Abarn$}}
\end{align}
% 

\paragraph{Representation and function class:}
$\gF\subseteq\{f:\Xaug \rightarrow \R^{k}\} \equiv \{F\in\R^{\Xaug \times k}\}$ is the function class for representation.
For any representation $f\in\gF$, we denote the normalized representation $\fn$ as $\fn(\bar{x}) = \sqrt{P(\bar{x})} f(\bar{x})$; for the matrix version $F\in\gF$, the normalized representation can be expressed as $\Fn = D^{\half} F$.
We denote the class of {\em normalized} representations as $\gFn = \left\{D^{\half} F \mid F\in\gF\right\}$.
There is a bijection between $\gF$ and $\gFn$ due to $D$ being full rank.
%

\paragraph{Downstream task:}
We are interested in a classification task on the original images $\Xorig$.
Let $g^{\star}\in\R^{\Xorig}$ be the ground truth labels on original images that is normalized to 1 \dipendra{how is  $\sum_{\bar{x}} g^\star(\bar{x}) = 1?$}
\ns{The $\ell_2$ norm is 1, so $\sum_{\bar{x}} g^{\star}(\bar{x})^2 = 1$.}\dipendra{Hmm..we have $\sum_{\bar{x}} g^\star(\bar{x})^2 = \sum_{\bar{x}} P(\bar{x}) y^\star(\bar{x})^2 = \sum_{\bar{x}, y(\bar{x})=1} P(\bar{x})$. Why would this be 1? Because labels are balanced? If yes, we should state this.}
\begin{align}
    g^{\star}(\bar{x}) = \sqrt{P(\bar{x})}~y^{\star}(\bar{x});~g^{\star} = \bar{D} \bm{y^{\star}}
\end{align}
The classification loss for a representation $F\in\gF$ is defined as
\begin{align}
    \Lclf(f) = \Lclf(F)
    &= \inf_{w\in\R^{k}} \ex_{\bar{x}} \left(\ex_{x\mid\bar{x}}[f(x)|\bar{x}]^{\top} w - y^{\star}(\bar{x})\right)^2
    = \inf_{w\in\R^{k}} \left\|\bar{D}^{-\half}\Abar Fw - g^{\star}\right\|^2\\
    &= \inf_{w\in\R^{k}} \left\|\Abarn \Fn w - g^{\star}\right\|^2
    = \left\|P^{\perp}_{\Abarn \Fn} g^{\star}\right\|_F^2
    = 1 - \left\|P_{\Abarn \Fn} g^{\star}\right\|_F^2
\end{align}
We abuse notation and denote $\Lclf(\Fn) = \Lclf(F)$ and $\Lclf(\fn) = \Lclf(f)$.
%

\paragraph{Contrastive loss:}
For representation $f\in\gF$ or $F\in\gF$, the spectral contrastive loss is defined as
\begin{align}
    \Lspec(f)
    &= \Lspec(F)
    = -2\ex_{(x,x^{+})}\left[f(x)^{\top} f(x^{+})\right] + \ex_{x,x^{-}} \left[\left(f(x)^{\top} f(x^{-})\right)^2\right]\\
    &= \left\|D^{-\half} \A D^{-\half} - D^{\half} FF^{\top} D^{\half}\right\|_{F}^2 - \left\|D^{-\half} \A D^{-\half}\right\|_{F}^2\\
    &= \left\|\An - \Fn \Fn^{\top}\right\|_{F}^2 - \left\|\An\right\|_{F}^2
    = \left\|\Abarn^{\top}\Abarn - \Fn \Fn^{\top}\right\|_{F}^2 - \left\|\An\right\|_{F}^2\\
    &= -2~\tr\left(\Abarn^{\top}\Abarn\Fn\Fn^{\top}\right) + \left\|\Fn \Fn^{\top}\right\|_{F}^2
    \label{old_eqn:contrastive_loss_simplified}
\end{align}


We make the following assumption about the function class $\gF$ (\ns{may or may not be needed})
\begin{assumption}
\label{old_asmp:closed_fn_class}
    Let $P_{\Abarn} = \Abarn^{\dagger} \Abarn \in \R^{\Xaug \times \Xaug}$ be the projection matrix for rows of $\Abarn$. We assume that the function class $\gFn$ is closed under the project by $\Abarn$, i.e. $P_{\Abarn} \gFn \coloneqq \left\{P_{\Abarn} \Fn \mid \Fn \in \gFn\right\} \subseteq \gFn$.
    In other words, for every $F\in\gF$, $D^{-\half} P_{\Abarn} D^{\half} F \in \gF$
\end{assumption}



%%%%%%%% Kernel result
\paragraph{Result for kernel based function class:}

We state the result for a linear representation function class and when $\A$ is block identity and previous analyses are vacuous.
We say $\A$ is a block identity matrix if the augmentation distribution for each image $\bar{x}$ is a uniform distribution over $|\Xaug|/|\Xorig|$ augmentations.

Let $\Phi\in\R^{\Xaug\times D}$ be representations with $K = \Phi \Phi^{\top} \in \R^{\Xaug \times \Xaug}$ be the corresponding kernel on augmentations.
The function class of interest is $\gF_{B} = \left\{\Phi W \mid W\in\R^{D\times k}, \|W\|^2_{F} \le B \right\}$.
Denote $\gF_{\infty} = \left\{\Phi W \mid W\in\R^{D\times k}\right\}$ to be the unconstrained linear representation class.
Note that when $\Phi$ is full row rank then $\gF_{\infty}$ contains all $k$-dimensional representation functions.

Denote $\Phi_{\norm} = D^{\half} \Phi$ and $K_{\norm} = \Phi_{\norm} \Phi_{\norm}^{\top}$ to be the normalized versions.
Define the augmented kernel $\bar{K}_{\norm} = \Abarn K_{\norm} \Abarn^{\top} \in \R^{\Xorig \times \Xorig}$ on the original images by using features of an image $\bar{x}$ as the average feature of its augmentations. For the first result we will make the following {\color{red} assumption} about the kernel $K_{\norm}$.
\begin{assumption}
\label{old_asmp:kernel_augmentation_commutative}
    Let $P_{\Abarn} = \Abarn^{\dagger} \Abarn \in \R^{\Xaug \times \Xaug}$ be the projection matrix for rows of $\Abarn$.
    We assume that $P_{\Abarn}$ commutes with $K_{\norm}$, i.e. $P_{\Abarn} K_{\norm} = K_{\norm} P_{\Abarn}$.
\end{assumption}
\ns{This assumption is kind of weird, but need it for some technical reasons currently. The result without this assumption will actually be more interesting, but also more complicated to prove.}

\begin{lemma}
    % Let $B = \inf \{B'\in\R \mid f^{\star}\in\gF_{B'}\}$ contains an optimal solution of $\Lspec$.
    Let $B$ be the smallest $B'\in\R$ such that contains $\gF_{B'}$ contains a minimizer of $\Lspec$.
    \ns{Smallest function class of the form $\gF_{B}$ that can minimize contrastive loss.}
    Let $\lambda_{1}, \dots, \lambda_{|\Xorig|} \in \R$ be the eigenvalues of $\bar{K}^{-1}$ from smallest to largest.
    Then under \Cref{asmp:kernel_augmentation_commutative}, any $\epsilon$-optimal representation $f$ within the class $\gF_{B}$, i.e. $\Lspec(f) - \inf\limits_{f^{\star}\in\gF_{B}} \Lspec(f^{\star}) \le \epsilon$, will satisfy
    \begin{align*}
        \Lclf(f) \le \min_{1 \le k' \le k} \left\{\frac{B^{\star} - \lambda_{1}}{\lambda_{k'+1} - \lambda_{1}} + 2 \frac{\sum_{i=1}^{k} \lambda_{i}}{\lambda_{k+1} - \lambda_{k'}} \sqrt{\frac{\epsilon}{k}}\right\}
    \end{align*}
    where $B^{\star} = {g^{\star}}^{\top} \bar{K}^{-1} g^{\star}$ is the norm of linear classifier need to fit $g^{\star}$ using features $\Phi$.
\end{lemma}
\ns{Similar statement can probably be shown for even smaller values of $B$. The transfer bound can be vacuous for much larger value of $B$. There also exists another representation such that no norm bound can lead to non-vacuous transfer bound even though there exists a good function in the class.}

\ns{The bound looks similar to the spectral contrastive bound, except the eigenvalues and gaps are based on the function class kernel, and the $\alpha$ is replaced by $B^{\star}$.}



\begin{proof}

    We will mostly refer to normalized adjacency matrices $\An = D^{-\half} A D^{-\half}$, $\Abarn = \bar{D}^{-\half} \Abar D^{-\half}$ and normalized representation $\Fn = D^{\half} F$.
    Our interest is in lower bounding
    \begin{align}
        \trf_{\gF}(\beta)
        &= \kappa(\beta) - \kappa(0)\text{, where}\\
        \kappa(\beta)
        &= \inf_{\substack{\Lclf(\Fn) \ge \beta\\\Fn\in\gFn}} \Lspec(\Fn)
    \end{align}
    So we start with trying to find an expression for $\kappa(\beta)$, for which we will use the following lemma.
    \begin{lemma}
    \label{old_lem:general_bound}
        For any function class $\gF$, define the function class $C\gF = \left\{CF \mid F\in\gF\right\}$ for any matrix $C$. Let $\gK(\gF) = \left\{F F^{\top} \mid F\in\gF\right\}$ be the set of kernels expressible by representations from a class $\gF$.
        Under \Cref{asmp:closed_fn_class}, we have the transfer bound $\trf_{\gF}(\beta)
        = \kappa(\beta) - \kappa(0)$, where 
        \begin{align*}
            \kappa(\beta)
            = ~&\inf_{\{\sigma_{i}\}_{i=1}^{k}, \{h_{i}\}_{i=1}^{k}} -2~\sum_{i=1}^{k} \sigma_{i} + \sum_{i,j} \sigma_{i} \sigma_{j} (h_{i}^{\top} \An^{\dagger} h_{j})^2\\
            \text{s.t.}~
            &\sum_{i} \sigma_{i} h_{i} h_{i}^{\top} \in \gK(\Abarn \gFn),~~~~
            \left\|(\sum_{i} h_{i} h_{i}^{\top}) g^{\star}\right\|_{F}^2 \le 1-\beta,\\
            & \sigma_{i} \ge 0,~~~~
            h_{i}^{\top} h_{j} = \bm{1}_{i = j}
        \end{align*}
    \end{lemma}
    We will prove this lemma later, but we instantiate it for the current setting.
    In order to invoke \Cref{lem:general_bound}, we first need to show that \Cref{asmp:closed_fn_class} holds for the current setting, for which we will use \Cref{asmp:kernel_augmentation_commutative}.
    We need to show that $P_{\An} \Fn \in \gFn$ when $\Fn \in \gFn$.
    For the current setting, $\gFn = \left\{\Phi_{\norm} W \mid W\in\R^{D\times k}, \|W\|^2_{F} \le B \right\}$.
    An alternate way to express the function class is $\gFn = \left\{\Fn\in\R^{\Xaug \times k} \mid \tr\left(\Fn^{\top} K_{\norm}^{-1} \Fn \right) \le B \right\}$.
    So for any $\Fn \in \gFn$,
    \begin{align*}
        B
        &\ge \tr\left(\Fn^{\top} K_{\norm}^{-1} \Fn \right)
        = \tr\left(\Fn^{\top} (P_{\An} + P^{\perp}_{\An}) K_{\norm}^{-1} (P_{\An} + P^{\perp}_{\An}) \Fn \right)\\
        &= \tr\left(\Fn^{\top} P_{\An} K_{\norm}^{-1} P_{\An} \Fn \right) + 2~\tr\left(\Fn^{\top} P_{\An} K_{\norm}^{-1} P^{\perp}_{\An} \Fn \right) + \tr\left(\Fn^{\top} P^{\perp}_{\An} K_{\norm}^{-1} P^{\perp}_{\An} \Fn \right)\\
        &=^{(a)} \tr\left(\Fn^{\top} P_{\An} K_{\norm}^{-1} P_{\An} \Fn \right) + 2~\tr\left(\Fn^{\top} K_{\norm}^{-1} P_{\An} P^{\perp}_{\An} \Fn \right) + \tr\left(\Fn^{\top} P^{\perp}_{\An} K_{\norm}^{-1} P^{\perp}_{\An} \Fn \right)\\
        &= \tr\left(\Fn^{\top} P_{\An} K_{\norm}^{-1} P_{\An} \Fn \right) + \tr\left(\Fn^{\top} P^{\perp}_{\An} K_{\norm}^{-1} P^{\perp}_{\An} \Fn \right)
        \ge \tr\left(\Fn^{\top} P_{\An} K_{\norm}^{-1} P_{\An} \Fn \right)
    \end{align*}
    where $(a)$ uses the commutativity property from \Cref{asmp:kernel_augmentation_commutative}.
    
    Having shown that \Cref{asmp:closed_fn_class} is satisfied, we can invoke \Cref{lem:general_bound}.
    It can be shown that for this setting, $\An = I_{\Xorig}$, and $\gK(\Abarn \gFn) = \left\{M\in\R^{\Xorig\times\Xorig} \mid tr(M^{\top} \bar{K}_{\norm}) \le B\right\}$.
    % $\gK(\Abarn \gFn) = \left\{\Abarn\Phi_{\norm}WW^{\top}\Phi_{\norm}^{\top}\Abarn^{\top} \mid \|W\|_{F}^2 \le B\right\}$.
    Thus the optimization problem for $\kappa(\beta)$ from \Cref{lem:general_bound} reduces to
    \begin{align*}
        \kappa(\beta)
        = ~&\inf_{\bm{\sigma}, \{h_{i}\}_{i=1}^{k}} -2~\bm{\sigma}^{\top} \bm{1} + \|\bm{\sigma}\|^2 = \inf_{\bm{\sigma}, \{h_{i}\}_{i=1}^{k}} -k + \|\bm{1} - \bm{\sigma}\|^2\\
        \text{s.t.}~
        &\sum_{i} \sigma_{i} ~h_{i}^{\top} \bar{K}_{\norm} h_{i} \le B,~~~~
        \sigma_{i} \ge 0,\\
        & \left\|(\sum_{i} h_{i} h_{i}^{\top}) g^{\star}\right\|_{F}^2 \le 1-\beta,~~~~
        h_{i}^{\top} h_{j} = \bm{1}_{i = j}
    \end{align*}
    We first consider the minimization over $\bm{\sigma}$ for a fixed $k$-dimensional subspace $\{h_{i}\}$.
    The minimization reduces to
    \begin{align*}
        \inf_{\bm{\sigma}} \left\{-k + \|\bm{1} - \bm{\sigma}\|^2\right\}~~
        \text{s.t.}~~
        \bm{\sigma}^{\top} \rho \le B,~~
        \bm{\sigma} \ge 0
    \end{align*}
    where $\rho = (h_{i}^{\top} \bar{K}_{\norm} h_{i})_{i=1}^{k} \in \R^{k}$.
    Firstly we note that the unconstrained optimal value of this is obtained at $\bm{\sigma}=\bm{1}$.
    This can be achieved when the constraint $\bm{1}^{\top} \rho \le B$.
    The smallest value of $B$ for which this is possible is $\sum_{i=1}^{k} \sigma_{i} h_{i}^{\top} \bar{K}_{\norm} h_{j} \ge \sum_{i=1}^{k} \lambda_{i}$, which is achievable by picking $h_{i}$ to be the $i^{th}$ eigen-vector of $\bar{K}_{\norm}$.
    Thus $B = \sum_{i=1}^{k} \lambda_{i}$ and $\kappa(0) = 0$.
    Back to the minimization; looking at the Lagrangian gives us that $\kappa(\beta) \ge \frac{\left(\bm{1}^{\top} \rho - B\right)^2}{\|\rho\|^2}$.

    \ns{We will then argue that firstly the bottom $k$ eigen-vectors of $\bar{K}_{\norm}$ capture a lot of mass of $g^{\star}$ by virtue of $g^{\star} \bar{K}_{\norm}^{-1} g^{\star}$ being small. Next using the above expression for $\kappa(\beta)$ it can be shown that sub-optimality in contrastive loss means that we are far enough from the bottom $k$ eigen-vectors of $\bar{K}_{\norm}$, thus leading to the final transfer bound.}

\end{proof}

\begin{proof}[Proof of \Cref{lem:general_bound}]
    We will mostly refer to normalized adjacency matrices $\An = D^{-\half} A D^{-\half}$, $\Abarn = \bar{D}^{-\half} \Abar D^{-\half}$ and normalized representation $\Fn = D^{\half} F$.
    Our interest is in lower bounding
    \begin{align}
        \trf_{\gF}(\beta)
        &= \kappa(\beta) - \kappa(0)\text{, where}\\
        \kappa(\beta)
        &= \inf_{\substack{\Lclf(\Fn) \ge \beta\\\Fn\in\gFn}} \Lspec(\Fn)
    \end{align}
    So we start with trying to find an expression for $\kappa(\beta)$.

    {\bf Step 1:}
    Notice that for any $\Fn\in\gFn$ we have the following 3 properties: (a) $P_{\An} \Fn \in \gFn$ (from \Cref{asmp:closed_fn_class}), (b) $\Lspec(P_{\An} \Fn) \le \Lspec(\Fn)$, (c) $\Lclf(P_{\An} \Fn) = \Lclf(\Fn)$.
    So to compute $\kappa(\beta)$, we can only consider normalized representations $\Fn$ that are in the span of $\Abarn$, i.e. $P_{\Abarn}\Fn = \Fn$, since it only makes the contrastive loss small without affecting the classification loss.
    We have reduced the problem to
    \begin{align*}
        \kappa(\beta)
        = ~&\inf_{\Fn} \Lspec(\Fn)\\
        \text{s.t.}~
        &\Fn \in \gFn,~
        P_{\Abarn}\Fn = \Fn\\
        &\Lclf(\Fn) \ge \beta
    \end{align*}
    %
    {\bf Step 2:}
    For some reason, we start by assuming that $\bm{\sigma} = \{\sigma_i\}_{i=1}^{k}$ are the singular values and $\{h_{i}\}_{i=1}^{k}$ are the left singular vectors of $\Abarn \Fn \in \R^{\Xorig \times k}$.
    This gives us the following
    \begin{align}
        \left(\Abarn \Fn\right)\left(\Abarn \Fn\right)^{\top}
        &= \sum_{i=1}^{k} \sigma_{i} h_{i} h_{i}^{\top}~
        \text{ and }P_{\Abarn \Fn}
        = \sum_{i=1}^{k} h_{i} h_{i}^{\top}\\
        \text{where }~\{h_{i}\}_{i=1}^{k}~
        &\text{ satisfy }h_{i}^{\top} h_{j} = \bm{1}_{i=j}
    \end{align}
    Since $\Fn$ lies in the span of $\Abarn$ from step 1, we also get the following
    \begin{align}
        \Fn \Fn^{\top} = \sum_{i=1}^{k} \sigma_i \Abarn^{\dagger} h_{i} h_{i}^{\top} (\Abarn^{\dagger})^{\top}
    \end{align}
    %
    Using this decomposition, we can express the contrastive and downstream losses as follows
    \begin{align*}
        \Lspec(\Fn)
        % = \Lspec(\{h_{i}\}, \bm{\sigma})
        &= -2~\tr\left(\Abarn^{\top}\Abarn\Fn\Fn^{\top}\right) + \left\|\Fn\Fn^{\top}\right\|_{F}^2\\
        &= -2~\tr\left(\sum_{i} \sigma_{i} h_{i} h_{i}^{\top}\right) + \left\|\sum_{i}\sigma_{i} \Abarn^{\dagger} h_{i} h_{i}^{\top} (\Abarn^{\dagger})^{\top}\right\|_{F}^2\\
        &= -2\sum_{i} \sigma_{i} + \sum_{i,j} \sigma_{i} \sigma_{j} \left(h_{i}^{\top} (\Abarn^{\dagger})^{\top} \Abarn^{\dagger} h_{j}\right)
        = -2\sum_{i} \sigma_{i} + \sum_{i,j} \sigma_{i} \sigma_{j} \left(h_{i}^{\top} \An^{\dagger} h_{j}\right)\\
        &= -2~\bm{\sigma}^{\top} \bm{1} + \bm{\sigma}^{\top} \Lambda \bm{\sigma}
    \end{align*}
    where $\Lambda\in\R^{k\times k}$ has entries $\Lambda(i,j) = h_{i}^{\top} \An^{\dagger} h_{j}$.
    The classification loss can be rewritten as
    \begin{align}
        \Lclf(\Fn)
        = 1 - \left\|P_{\Abarn \Fn} g^{\star}\right\|_{F}^2
        = 1 - \left\|\left(\sum_{i=1}^{k} h_{i} h_{i}^{\top}\right) g^{\star}\right\|_{F}^2
    \end{align}
    The minimization problem for $\kappa(\beta)$ then reduces to the following
    %
    To do the minimization for the computation of $\kappa(\beta)$, we will separate the minimization over $\bm{\sigma} = (\sigma_{i})_{i=1}^{k}$ and $\{h_{i}\}_{i=1}^{k}$.
    % We are thus implicitly making the following assumption
    % \begin{assumption}
    % \label{old_asmp:separate}
    %     For every orthonormal basis $\{h_{i}\}_{i=1}^{k}$ of rank $k$ that can be expressed as $\Abarn \Fn$ for $\Fn\in\gFn$, for every $\bm{\sigma}\in\R^{k}$, $\sum_{i=1}^{k} \sigma_{i} h_{i} h_{i}^{\top}$ can also be expressed as $\Abarn \Fn'$ for $\Fn'\in\gFn$.
    %     \ns{This is satisfied if a linear projection layer is added on top of the representation.}
    % \end{assumption}

    Let $\gK(\gF) = \left\{F F^{\top} \mid F\in\gF\right\}$ be the set of kernels expressible by representations from a class $\gF$.
    Also define the function class $C\gF = \left\{CF \mid F\in\gF\right\}$ for any matrix $C$.
    The minimization problem can now be further reduced to the following
    \begin{align*}
        \kappa(\beta)
        = ~&\inf_{\bm{\sigma}, \{h_{i}\}_{i=1}^{k}} -2~\bm{\sigma}^{\top} \bm{1} + \bm{\sigma}^{\top} \Lambda \bm{\sigma}\\
        \text{s.t.}~
        &\sum_{i}\sigma_{i} \left(\Abarn^{\dagger} h_{i} h_{i}^{\top} (\Abarn^{\dagger})^{\top}\right) \in \gK(\gFn)
        \equiv
        \sum_{i} \sigma_{i} h_{i} h_{i}^{\top} \in \gK(\Abarn \gFn),\\
        & \left\|(\sum_{i} h_{i} h_{i}^{\top}) g^{\star}\right\|_{F}^2 \le 1-\beta\\
        & \bm{\sigma} \ge 0
    \end{align*}
\end{proof}


\iffalse

\paragraph{Special case:} For the kernel function class, the above optimization reduces to
\begin{align*}
    \kappa(\beta)
    = ~&\inf_{\bm{\sigma}, \{h_{i}\}_{i=1}^{k}} -2~\bm{\sigma}^{\top} \bm{1} + \bm{\sigma}^{\top} \Lambda \bm{\sigma}\\
    \text{s.t.}~
    &\sum_{i} \sigma_{i} h_{i}^{\top} K^{-1} h_{i} \le B, ~\bm{\sigma} \ge 0\\
    & \left\|\left(\sum_{i} h_{i} h_{i}^{\top}\right) g^{\star}\right\|_{F}^2 \le 1-\beta
\end{align*}
Doing minimization over $\bm{\sigma}$ will give the following
\ns{Issue with the steps below. Need to add constraint that $\sigma_{i} > 0$. This can change the objective...}
\begin{align*}
    \kappa(\beta)
    = ~&\inf_{\{h_{i}\}_{i=1}^{k}} -\bm{1}^{\top} \Lambda^{-1} \bm{1} + \frac{\left(\rho^{\top}\Lambda^{-1}\bm{1} - B\right)_{+}^2}{\rho^{\top}\Lambda^{-1} \rho}\\
    \text{s.t.}~
    & \left\|\left(\sum_{i} h_{i} h_{i}^{\top}\right) g^{\star}\right\|_{F}^2 \le 1-\beta\\
    &\rho_{i}
    = h_{i}^{\top} \tilde{K}^{-1} h_{i}
\end{align*}
where $\Lambda_{i,j} = \left(h_{i}^{\top} \Abarn^{-1} h_{j}\right)^2$

\fi


\iffalse
\paragraph{Back to block identity:}
Here $\Lambda = I$, so problem reduces to
\begin{align*}
    \kappa(\beta)
    = ~&\inf_{\{h_{i}\}_{i=1}^{k}} \frac{\left(\rho^{\top}\bm{1} - B\right)_{+}^2}{\left\|\rho\right\|^2}\\
    \text{s.t.}~
    & \left\|\left(\sum_{i} h_{i} h_{i}^{\top}\right) g^{\star}\right\|_{F}^2 \le 1-\beta\\
    &\rho_{i}
    = h_{i}^{\top} \tilde{K}^{-1} h_{i}
\end{align*}
Can be reduced to minimization over the $k$-dimensional subspace $H\in\R^{\Xorig\times k} = [h_{1}, \dots, h_{k}]$.
Let $K(H) = H^{\top} K^{-1} H$, then the problem reduces to
\begin{align*}
    \kappa(\beta)
    = ~&\inf_{H\in\R^{\Xorig\times k}} \frac{\left(\tr\left(K(H)\right) - B\right)_{+}^2}{\left\|K(H)\right\|_F^2}\\
    \text{s.t.}~
    & \left\|H^{\top} g^{\star}\right\|^2 \le 1-\beta\\
    & H^{\top} H = I_{k}
\end{align*}
% So the transfer bound for the constrained optimization problem reduces to finding the transfer bound for the above objective
% \begin{align*}
%     L(H) = \frac{\left(\tr\left(H^{\top} K^{-1} H\right) - B\right)_{+}^2}{\left\|H^{\top} K^{-1} H\right\|_F^2}
% \end{align*}
\fi









\iffalse
\ns{===== This is incomplete ======

We will now recover the results from (HaoChen et al. 2020) for a general augmentation graph $\A$ that is not block identity.
For now we ignore the effect of function class.
%
\begin{prop}
    Let $\gamma_{i}$ be the $i^{th}$ largest eigenvalue of $\An$ and let $\lambda_{i} = 1-\gamma_{i}$
    Suppose the image-augmentation graph aligns with labels $g^{\star}$, i.e. $\|g^{\star} - \Abarn g^{\star}\| \le \alpha$. \ns{can be replaced with augmentation Bayes error from spectral conmtrastive learning paper, or some nearest-neighbor interpretation.}
    For any augmentation graph $\A$, we have
    \begin{align}
        \trf(\beta) \ge \left(\gamma_{k}^2 - \gamma_{k+1}^2\right) \left(\beta - \frac{\alpha}{1-\gamma_{k+1}}\right)_{+}
    \end{align}
    This gives the following guarantee for $\epsilon$ optimal representations $f$
    \begin{align}
        \Lclf(f) \le \frac{\alpha}{1-\gamma_{k+1}} + \frac{\epsilon}{\gamma_{k}^2 - \gamma_{k+1}^2}
    \end{align}
\end{prop}
}
%
\fi





\subsection{Random ideas}

Something about the minimum norm ERM on samples as the norm bound.

Style vs content view.

Train classifier in the "direction" of color jitter or gray scale. How can this be done?

How does final representation depend on initialization?

Evaluate SSL loss on GAN images.

Iterative sampling of patches and smoothing out steps.

Topic model kind of example. Perhaps masking of tokens, bag-of-ngram representations.

Image is composed of different factors of variation, augmentations attenuate some of the factors.

Move in direction of dog 1 to dog 2, compare to dog 1 and its augmentation .


Topic model example, with bigram representation. Possibly ngram generative model for text

Replacing words with POS tags

Gaussian blur + conv avg pool architecture make sense, because patches kind of look like independently sampled. Dictionary learning on blurred patches might give something.


